A Category Theoretic Interpretation of Gandy's Principles for Mechanisms

Based on Gandy's principles for models of computation we give category-theoretic axioms describing locally deterministic updates to finite objects. Rather than fixing a particular category of states, we describe what properties such a category should have. The computation is modelled by a functor that encodes updating the computation, and we give an abstract account of such functors. We show that every updating functor satisfying our conditions is computable.

==> eptcsdata.tex <==
\providecommand{\firstpage}{85}
\providecommand{\publicationstatus}{S. Alves and M. Pagani (Eds.): DCM 2018 and ITRS 2018\\
EPTCS 293, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.293.7}{10.4204/EPTCS.293.7}}
\pdfoutput=1

